GBOSE: Generalized Bandit Orthogonalized Semiparametric Estimation

In sequential decision-making scenarios i.e., mobile health recommendation systems revenue management contextual multi-armed bandit algorithms have garnered attention for their performance. But most of the existing algorithms are built on the assumption of a strictly parametric reward model mostly linear in nature. In this work we propose a new algorithm with a semi-parametric reward model with state-of-the-art complexity of upper bound on regret amongst existing semi-parametric algorithms. Our work expands the scope of another representative algorithm of state-of-the-art complexity with a similar reward model by proposing an algorithm built upon the same action filtering procedures but provides explicit action selection distribution for scenarios involving more than two arms at a particular time step while requiring fewer computations. We derive the said complexity of the upper bound on regret and present simulation results that affirm our methods superiority out of all prevalent semi-parametric bandit algorithms for cases involving over two arms.

==> lemmas and proofs/lemma10.tex <==


% \textbf{\begin{flalign*}
% &=2C^2\log\left(\frac{1}{\delta}\sqrt{\frac{C^{2d}det(B)}{C^{2d}det(\lambda I)}}\right)&\\
% &=2C^2\log\left(\frac{1}{\delta}\sqrt{\frac{det(B)}{det(\lambda I)}}\right)&\\
% &=2C^2\log\left(\frac{1}{\delta}\sqrt{\frac{(det(B)^{1/d})^d}{\lambda^d}}\right)&\\
% &\leq 2C^2\log\left(\frac{1}{\delta}\sqrt{\frac{(\lambda + \frac{T}{d})^d}{\lambda^d}}\right)
% \end{flalign*}
% \begin{flalign*}
% &=2C^2\log\left(\frac{1}{\delta}\sqrt{\left(\frac{(\lambda + \frac{T}{d})}{\lambda}\right)^d}\right)& \\
% &=2C^2\log\left(\frac{1}{\delta}\sqrt{\left(1 + \frac{T}{\lambda d}\right)^d}\right)&\\
% &=2(3)^2\log\left(\frac{1}{\delta}\sqrt{\left(1 + \frac{T}{\lambda d}\right)^d}\right)&\\
% &=18\log\left(\frac{1}{\delta}\sqrt{\left(1 + \frac{T}{\lambda d}\right)^d}\right)&\\
% &=18\log\left(\sqrt{\left(1 + \frac{T}{\lambda d}\right)^d}\right)+18\log\left(\frac{1}{\delta}\right)&\\
% &=18\log\left(1 + \frac{T}{\lambda d}\right)^{\frac{d}{2}}+18\log\left(\frac{1}{\delta}\right)&\\
% &=9d\log\left(1 + \frac{T}{\lambda d}\right)+18\log\left(\frac{1}{\delta}\right)&\\
% \end{flalign*}
% }

==> lemmas and proofs/lemma3.tex <==
$det(B)^{\frac{1}{d}} \leq \frac{1}{d}tr(B)
                    =\frac{1}{d}tr(\lambda I) + \frac{1}{d}tr\left(\sum X_{i}X_{i}^T\right)
                     =\frac{1}{d}tr(\lambda I) + \frac{1}{d}tr\left(\sum_{i=1}^{T} \Vert b_i \Vert_{2}^{2}\right)
                     \leq \lambda + \frac{TL^2}{d} = \lambda + \frac{T}{d}$


==> lemmas and proofs/sub_proof2.tex <==
\newpage
\textbf{**Text \cite{DELAPENA20094210}**}
$$D_t^{\lambda} \triangleq  \exp\big( \langle \lambda, X_t, \zeta_t \rangle - \frac{C^2 \langle \lambda, X_t \rangle^2}{2} \big).$$

\textbf{** Observe part $\mathbb{E}(D_t^{\lambda} | \mathcal{F}_t) \leq 1$ **}

\begin{align*}
    \mathbb{E}(D_t^{\lambda} | \mathcal{F}_t) &= \mathbb{E}[\mathbb{E}(D_t^{\lambda} | \mathcal{F}_t, \zeta_t) | \mathcal{F}_t] \\ 
    &= \mathbb{E}\Big[\mathbb{E} \big[ \exp\big( - \frac{C^2 \langle \lambda, X_t \rangle^2}{2}\big) \times \frac{1}{2} (\exp ( \langle \lambda, X_t \zeta_t \rangle ) + \exp ( - \langle \lambda, X_t \zeta_t \rangle )) | \mathcal{F}_t, \zeta_t \big] | \mathcal{F}_t \Big] \\
    &= \mathbb{E}\Big[\mathbb{E} \big[ \exp\big( - \frac{C^2 \langle \lambda, X_t \rangle^2}{2}\big) \times \cosh(\langle \lambda, X_t \zeta_t \rangle) | \mathcal{F}_t, \zeta_t \big] | \mathcal{F}_t \Big] \\
    &\leq \mathbb{E}\Big[\mathbb{E} \big[ \exp\big( - \frac{C^2 \langle \lambda, X_t \rangle^2}{2} + \frac{\langle \lambda, X_t \zeta_t \rangle^2}{2}\big) | \mathcal{F}_t, \zeta_t \big] | \mathcal{F}_t \Big] \leq 1.
\end{align*}
\textbf{** This Argument part**}
\begin{equation}
    \mathbb{E} [U_t^\lambda] = \mathbb{E} [U_{t-1}^\lambda \mathbb{E}[D_t^\lambda | \mathcal{F}_t]] \leq \mathbb{E}[U_{t-1}^\lambda] \leq \dots \leq 1.
\end{equation}

==> tab/comparison.tex <==
\begin{table*}[ht]
\caption{Comparison of the other three semiparametric contextual MAB algorithms with GBOSE}
\resizebox{\linewidth}{!}{
\begin{tabular}{lllll}
\hline
\textbf{Properties} & Action-Centered TS & Semi TS & BOSE & GBOSE \\ \hline
Restriction on optimal policy           &     $\pi^{*}_{\overline{a}^*(t)} \in [p_{min}, p_{max}]$               &    None     & None      &    None   
\\
Derivation of $\pi(t)$           &     from $\tilde{\mu}(t)$               &from $\tilde{\mu}(t)$     &  Not specified when $N > 2$      &  from  $\tilde{\mu}(t)$   \\
Number of computations          &      $O(T)$              &    $O(NT)$     &  $O(N^2T)$    &   $O(N^2T)$    \\
Tuning parameters        &          $v$          &   $v$       &  $\lambda$ and $\gamma$     &     $\lambda$ and $\gamma$  
\\
$R(T)$           &    $O(Md^\frac{3}{2}\sqrt{T}\sqrt{log(T/\delta)^3})$                &      $O(d^\frac{3}{2}\sqrt{T}\sqrt{log(T/\delta)^3})$   &   $O(d\sqrt{T}log(T/\delta))$   &      $O(d\sqrt{T}log(T/\delta))$ \\ \hline
\end{tabular}
}
\end{table*}
